MM-OVSeg:Multimodal Optical-SAR Fusion for Open-Vocabulary Segmentation in Remote Sensing

Open-vocabulary segmentation enables pixel-level recognition from an open set of textual categories, allowing generalization beyond fixed classes. Despite great potential in remote sensing, progress in this area remains largely limited to clear-sky optical data and struggles under cloudy or haze-contaminated conditions. We present MM-OVSeg, a multimodal Optical-SAR fusion framework for resilient open-vocabulary segmentation under adverse weather conditions. MM-OVSeg leverages the complementary strengths of the two modalities--optical imagery provides rich spectral semantics, while synthetic aperture radar (SAR) offers cloud-penetrating structural cues. To address the cross-modal domain gap and the limited dense prediction capability of current vision-language models, we propose two key designs: a cross-modal unification process for multi-sensor representation alignment, and a dual-encoder fusion module that integrates hierarchical features from multiple vision foundation models for text-aligned multimodal segmentation. Extensive experiments demonstrate that MM-OVSeg achieves superior robustness and generalization across diverse cloud conditions. The source dataset and code are available at https://github.com/Jimmyxichen/MM-OVSeg.

==> backup/1_introduction_20251102.tex <==
\section{Introduction}
\label{sec:intro}

% \par Open-vocabulary semantic segmentation for remote sensing images (OVRS) seeks to assign a land-cover label to each pixel in a remote sensing image from an unrestricted set, delineated by text descriptions. Unlike tradition semantic segmentation, OVRS models leverage the strong open-vocabulary recognition abilities of the pre-trained vision-language foundation models (VLMs) ,e.g., CLIP \cite{openclip2022}, to transfer image-text matching to dense prediction. Despite achieving significant advancements \cite{shan2024open,ye2025towards,li2025exploring}, OVRS remains highly challenging. One of the primary difficulties arises from the cloud and haze occlusions. Specifically, current works \cite{cao2024open,li2025exploring} are almost exclusively trained and evaluated on clear-sky optical remote sensing datasets, implicitly assuming unobstructed RGB inputs. However, cloud and haze occlusions are ubiquitous in the remote sensing scene and disrupt surface reflectance, which in turn causes pronounced accuracy drops for optical-only OVRS methods. An example of this performance gap is illustrated in Figure. \ref{fig:motivation}.
\textcolor{blue}{Open-vocabulary segmentation (OVS) aims to assign semantic labels to image regions using an open-ended set of textual categories, enabling recognition beyond the classes observed during training. In remote sensing (RS), OVS is significant as it facilitates flexible and scalable land-cover understanding across diverse geographical regions without the need for exhaustive pixel-level annotations. Compared with traditional semantic segmentation, which is constrained to a fixed and limited set of predefined classes, OVS demonstrates superior generalization and adaptability to novel or fine-grained categories commonly encountered in RS imagery.}

\textcolor{blue}{However, existing studies on OVS in the RS domain~\cite{cao2024open,shan2024open,li2025exploring} have been predominantly limited to optical RGB data. Moreover, these approaches typically assume clean, clear-sky imagery. In practice, RS observations are often affected by cloud or haze contamination, which severely degrades visibility and model performance. Consequently, current OVS methods struggle to recognize objects under cloudy conditions, as illustrated in Figure 1. Such limitations not only hinder time-sensitive applications, such as rapid disaster response, but also undermine long-term monitoring and analysis tasks that rely on consistent and reliable scene understanding.}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{sec/fig1.pdf}
    \caption{Vis: RGB v.s. RGB (Thick cloud) seg vs. RGB+SAR seg; data vs data w/ cloud vs RGB+SAR seg}
    \label{fig:motivation}
\end{figure}

\textcolor{blue}{In this work, we investigate OVS based on the fusion of optical and synthetic aperture radar (SAR) modalities. Leveraging both modalities offers complementary advantages, as optical images provide rich spectral and semantic cues, while SAR data penetrate clouds and capture structural information, enabling robust scene understanding under cloudy or adverse weather conditions.}




% \par In this work, we introduce Synthetic Aperture Radar (SAR) as a complementary modality to optical imagery, enabling OVRS models to remain robust under cloud and haze occlusions. Unlike optical imagery, SAR provides all‑weather, day–night observations that are largely insensitive to cloud cover. These unique advantages spurred SAR’s widespread use across remote sensing applications such as cloud removal \cite{huang2015cloud,xu2022glf} and change detection \cite{muro2019mapping} under cloud and haze occlusions. However, directly applying existing OVRS methods to SAR imagery presents significant challenges owing to the absence of strong SAR‑specific semantic priors and the substantial modality gap between optical appearance cues and SAR backscatter signatures. One of the primary obstacles is the lack of SAR domain priors. The pre-trained VLMs are predominantly trained on RGB image datasets, meaning SAR images fall outside the distribution of their training data. As a result, VLM's effectiveness diminishes for SAR imagery, which are typical in dense segmentation tasks. Additionally, the inherent semantic complexity of SAR images—often characterized by intricate textures and non-intuitive patterns—makes segmentation more challenging than that of natural optical imagery, thereby limiting the advancement of multimodal OVRS models.

% To address the above challenges, we propose MM-OVSeg, a novel multimodal open-vocabulary semantic segmentation framework, as shown in Figure. \ref{fig:fig2}. The core idea of our MM-OVSeg model lies in effectively integrating specialist remote sensing semantic priors with generalist CLIP. In order to achieve this goal, we propose a multimodal DINO module to capture the remote sensing semantic priors from the multimodal inputs. Our multimodal DINO module employs two parallel branches, DINO‑Optical for RGB and DINO‑SAR for SAR, to capture modality‑specific features concurrently. The DINO-RGB branch is pretrained on a large-scale remote sensing image semantic segmentation dataset LandDiscover50K \cite{ye2025towards} and serves as the specialist backbone for RGB image. The DINO-SAR branch is pretrained through knowledge distillation \cite{hinton2015distilling} from the DINO-RGB branch, aligning SAR representations with the RGB‑learned semantic space. Given the pretrained DINO-RGB branch and DINO-SAR branch, a multimodal feature fusion module (MFF) is further proposed to fuse the SAR features and RGB features produced by two branches. This multimodal specialist features are then integrated with general features produced by Clip model, achieving more accurate mask predictions.

% Recognizing the absence
% of datasets specifically designed for remote sensing cross-modal distillation, we developed RGBSAR-Distill, a dataset comprising 25,087 RGB-SAR image pairs. These image pairs are strictly co-registered, with the RGB images being cloud-free and haze-free.

\textcolor{blue}{However, incorporating SAR data introduces substantial challenges. On one hand, vision foundation models are predominantly trained on RGB imagery, while SAR images exhibit distinct backscattering characteristics and texture patterns, resulting in a pronounced domain gap between RGB and SAR representations. On the other hand, vision–language models like CLIP and ALIGN are primarily trained with image-level supervision, which limits their ability to produce accurate dense predictions required for segmentation tasks. This limitation becomes even more severe for SAR imagery, where the domain discrepancy further weakens the spatial correspondence between visual and textual representations. As a result, effectively encoding SAR data in a manner compatible with text-aligned RGB representations, while achieving robust multimodal fusion for OVS, remains an open and significant challenge.}

\textcolor{blue}{In this paper, we propose MM-OVSeg, a multimodal Optical–SAR fusion framework for robust open-vocabulary segmentation under cloudy conditions. The framework comprises two key components designed to address the above challenges. First, the Cross-Modal Unification (CMU) module leverages paired RGB–SAR data for cross-modal distillation, aligning SAR visual embeddings with RGB embeddings distilled from VFMs, thereby establishing a shared representation space that enables VFMs to effectively leverage SAR information. Second, the Dual-Encoder Fusion (DEF) module integrates the CLIP encoder (for global representations) and the DINO encoder (for dense, local representations) to extract complementary RGB and SAR features, which are subsequently fused and aligned with the CLIP text encoder to achieve open-vocabulary segmentation.}

 The main contributions of this paper are summarized as follows: 
 
 1) We advance the multimodal OVRS field along with a tailored dataset named RGBSAR-Distill, comprising 25,087 paired RGB-SAR images.

 2) We introduce a multimodal OVRS framework named MM-OVSeg, combining the generalist Clip image encoder with the specialist multimodal DINO module for capturing remote sensing semantic priors.

 3) Extensive experiments demonstrate that our MM-OVSeg outperforms existing state-of-the-art OVRS methods under cloud and haze occlusions.

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has only two authors.
% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}


==> backup/4_experiments_20251113.tex <==

\section{Experiments}
%--------------------------------
% \begin{table*}[t]
% \centering
% \caption{\label{tab:table1}{}}

% \resizebox{\linewidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline

% \scriptsize{\bf Dataset} & \scriptsize{\bf N\_category} & \scriptsize{Train Category} & \scriptsize{Unseen Category} & \scriptsize{\# Train} & \scriptsize{\# Test} 
% \\\hline
% \scriptsize{OpenEarthMap-SAR \cite{xia2025openearthmap} (thin / thick cloud)} & \scriptsize{8} & \scriptsize{[Bareland, Rangeland, Developed space, tree, Agriculture land]} & \scriptsize{[Road, water, building]} & \scriptsize{4,333} & \scriptsize{490} 
% \\\hline

% \scriptsize{PIE-RGB-SAR \cite{ZHANG2024574}} & \scriptsize{6} & \scriptsize{[backbroad, city, forest, farmland]} & \scriptsize{[Road, water]} & \scriptsize{2,433} & \scriptsize{2,432}
% \\\hline

% \scriptsize{DDHR-SK \cite{ren2022dual}} & \scriptsize{5} & \scriptsize{[Forest, City, Farmland]} & \scriptsize{[Road, water]} & \scriptsize{3,087} & \scriptsize{3,086} 

% \\\hline

% \scriptsize{DDHR-CH \cite{ren2022dual}} & \scriptsize{5} & \scriptsize{[Forest, City, Farmland]} & \scriptsize{[Road, water]} & \scriptsize{0} & \scriptsize{2,122}

% \\\hline
% \end{tabular}}
% \end{table*}

%--------------------------------
% \begin{table*}[t] %\color{red} % 删掉\color{red}即可，不加resizebox
%     \footnotesize % 这里整体调字体
%     \centering
%     \begin{tabular}{l|c|c|c|c|c}
%     \toprule
%         Dataset & N\_category & Train Category & Unseen Category & \# Train & \# Test \\
%     \midrule
%         PIE-RGB-SAR \cite{ZHANG2024574} & 6 & [backbroad, city, forest, farmland] & [Road, water] & 2,433 & 2,432 \\
 
%     \midrule
%         DDHR-SK \cite{ren2022dual} & 5 & [Forest, City, Farmland] & [Road, water] & 3,087 & 3,086 \\
%     \midrule
%         DDHR-CH \cite{ren2022dual} & 5 & [Forest, City, Farmland] & [Road, water] & 0 & 2,122 \\
%     \midrule
%         OEM-SAR \cite{xia2025openearthmap} & 8 & [Bareland, Rangeland, Developed space, tree, Agriculture land] & [Road, water, building] & 4,333 & 490 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Open-Vocabulary Setting for Four Datasets. OEM-SAR includes two subsets: OEM-SAR\textsuperscript{\#} (thick cloudy data) and OEM-SAR\textsuperscript{*} (thin cloudy data). ‘N\_category' indicates the number of the category. ‘\# Train' and ‘\# Test' denote the number of training samples and testing samples, respectively.}
%     \label{tab:table1}
% \end{table*}

% \begin{table*}[t]
%     \footnotesize
%     \centering
%     \begin{tabular}{cccc|cccc}
%     \toprule
%        \multicolumn{4}{c|}{Train} & \multicolumn{4}{c}{Test} \\
%        Dataset  & Categories & Cloudy & Real & Dataset  & Categories & Cloudy & Real \\
%     \midrule
%     % \midrule
%        PIE-Cloud & \textit{backbroad, city, forest, farmland} & \cmark & \cmark & PIE-Cloud & \textit{road, water}& \cmark & \cmark \\
%     \midrule
%        DDHR-SK & \textit{forest, city, farmland} & \cmark & \xmark & DDHR-SK & \textit{road, water}& \cmark & \xmark \\
%     % \midrule
%        OEM-SAR-Thick & \textit{Bareland, Rangeland, Developed space, tree, Agriculture land} & \cmark & \xmark & OEM-SAR-Thick & \textit{road, water, building}& \cmark & \xmark \\
%     % \midrule
%        OEM-SAR-Thin & \textit{Bareland, Rangeland, Developed space, tree, Agriculture land} & \cmark & \xmark & OEM-SAR-Thin & \textit{road, water, building}& \cmark & \xmark \\
%     \midrule
%        PIE-RGB & \textit{backbroad, city, forest, farmland} & \xmark & \xmark & PIE-RGB & \textit{road, water}& \xmark & \xmark \\
%     \midrule
%        DDHR-SK & \textit{forest, city, farmland} & \cmark & \xmark & DDHR-CH & \textit{road, water}& \cmark & \cmark \\
%     \bottomrule
%     \end{tabular}
%     \caption{Datasets for OVS.}
%     \label{tab:placeholder}
% \end{table*}

%--------------------------------
\begin{table*}[t] %\color{red}
    % \footnotesize % 这里整体调字体
    \setlength{\tabcolsep}{12pt}
    % \renewcommand{\arraystretch}{1.15}
    % \resizebox{\linewidth}{!}{%
    \centering
    \begin{tabular}{l|c|cccccc|c}
    \toprule
        Method & Publication & \ding{172} & \ding{173} & \ding{174} & \ding{175} & \ding{176} & \ding{177} & Mean \\
    \midrule
        CAT-Seg \cite{cho2024catseg} & CVPR'24 & 54.5 & 54.2 & 33.8 & 29.5  & 55.8 & 27.8 & 42.6\\

    % \midrule
        EBSeg \cite{shan2024open} & CVPR'24 & 50.8 & 51.1 & 27.2 & 25.6 & 51.0 & 26.7 & 38.7\\

    % \midrule
        GSNet \cite{ye2025towards} & AAAI'25 & 57.0 & 55.0 & 35.2 & 37.0 & 57.2 & 32.4 & 45.6\\

    % \midrule
       SegEarth-OV \cite{li2025segearth} & CVPR'25 & 45.1 & 17.6 & 28.9 & 18.5 & 51.8 & 24.2 & 31.0\\

    % \midrule
    %     RSKT-Seg \cite{li2025exploring} & Arxiv'25 & 56.8 & 68.5 & 36.0 & 37.7 & 35.4 & 57.2 & 48.6\\

    % \midrule
        FGA-Seg \cite{li2025fgaseg} & Arxiv'25 & 51.6 & 51.6 & 26.0 & 32.8 & 52.1 & 40.6 & 42.5\\
    % \midrule
        \textbf{MM-OVSeg (ours)} & -- & \textbf{57.7} & \textbf{73.1} & 
        \textbf{36.6} &
         \textbf{40.2} &  \textbf{59.7} & 
         \textbf{42.6} &
         \textbf{51.7} \\
    \bottomrule
    \end{tabular}
    \caption{Comparison of OVS methods across various evaluation settings as illustrated Table 1.
    \ding{172}: PIE-cloud→PIE-cloud; \ding{173}: DDHR-SK→DDHR-SK; \ding{174}: OEM-thick→OEM-thick; \ding{175}: OEM-thin→OEM-thin; \ding{176}: PIE-clean→PIE-clean; \ding{177}: DDHR-SK→DDHR-CH.}
    \label{tab:table2}
\end{table*}


%--------------------------------------
\begin{figure*}[t]
\centering
% \includegraphics[width=\linewidth]{sec/fig5.pdf}
\includegraphics[width=\linewidth]{Figures/Fig-PerClass.pdf}
%\begin{minipage}{0.8\textwidth}
\caption{{\bf Statistics of Open-Vocabulary Semantic Segmentation Per-class Results.} \ding{172}: PIE-cloud→PIE-cloud; \ding{173}: DDHR-SK→DDHR-SK; \ding{174}: OEM-thick→OEM-thick; \ding{175}: OEM-thin→OEM-thin; \ding{176}: PIE-clean→PIE-clean; \ding{177}: DDHR-SK→DDHR-CH. Please refer to Table 1 for dataset details.}
%\end{minipage}
\label{fig:figzhu}
\end{figure*}

%--------------------------------
% \begin{table*}[t] %\color{red}
%     % \footnotesize % 这里整体调字体
%     \setlength{\tabcolsep}{12pt}
%     % \renewcommand{\arraystretch}{1.15}
%     % \resizebox{\linewidth}{!}{%
%     \centering
%     \begin{tabular}{l|c|cccccc|c}
%     \toprule
%         Method & Publication & \ding{172} & \ding{173} & \ding{174} & \ding{175} & \ding{176} & \ding{177} & Mean \\
%     \midrule
%         CAT-Seg \cite{cho2024catseg} & CVPR'24 & 54.5 & 54.2 & 27.8 & 29.5 & 33.8 & 55.8 & 42.6\\

%     % \midrule
%         EBSeg \cite{shan2024open} & CVPR'24 & 50.8 & 51.1 & 26.7 & 25.6 & 27.2 & 51.0 & 38.7\\

%     % \midrule
%         GSNet \cite{ye2025towards} & AAAI'25 & 57.0 & 55.0 & 32.4 & 37.0 & 35.2 & 57.2 & 45.6\\

%     % \midrule
%        SegEarth-OV \cite{li2025segearth} & CVPR'25 & 45.1 & 17.6 & 24.2 & 18.5 & 28.9 & 51.8 & 31.0\\

%     % \midrule
%     %     RSKT-Seg \cite{li2025exploring} & Arxiv'25 & 56.8 & 68.5 & 36.0 & 37.7 & 35.4 & 57.2 & 48.6\\

%     % \midrule
%         FGA-Seg \cite{li2025fgaseg} & Arxiv'25 & 51.6 & 51.6 & 40.6 & 32.8 & 26.0 & 52.1 & 42.5\\
%     % \midrule
%         \textbf{MM-OVSeg (ours)} & -- & \textbf{57.7} & \textbf{73.1} & \textbf{42.6} & \textbf{40.2} & \textbf{36.6} & \textbf{59.7} & \textbf{51.7} \\
%     \bottomrule
%     \end{tabular}
%     \caption{Comparison of OVS methods across various evaluation settings as illustrated Table 1.
%     \ding{172}: PIE-cloud→PIE-cloud; \ding{173}: DDHR-SK→DDHR-SK; \ding{174}: DDHR-SK→DDHR-CH; \ding{175}: OEM-thin→OEM-thin; \ding{176}: OEM-thick→OEM-thick; \ding{177}: PIE-clean→PIE-clean.}
%     \label{tab:table2}
% \end{table*}
% -------- table1 ------------
% \begin{table*}[t]
% \centering
% \caption{\label{tab:table2}{{\bf Open-Vocabulary Semantic Segmentation Results on Four Datasets.} Mean IoU (\%) is used as the evaluation metric. ‘N\_category' indicates the number of the category. }}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|c|c|c|c|c|c|c}
% \htop

% \scriptsize{\bf Method} & \scriptsize{\bf VLM} & \scriptsize{\bf OpenEarthMap-SAR \cite{xia2025openearthmap} (thick cloud)} & \scriptsize{\bf OpenEarthMap-SAR \cite{xia2025openearthmap} (thin cloud)} & \scriptsize{\bf PIE-RGB-SAR \cite{ZHANG2024574}} & \scriptsize{\bf DDHR-SK \cite{ren2022dual}} & \scriptsize{\bf DDHR-CH \cite{ren2022dual}}  & \scriptsize{\bf Mean mIoU}  

% \\\hline
% \scriptsize{CAT-Seg \cite{cho2024catseg}} & \scriptsize{CLIP ViT-B/16} & \scriptsize{33.75} & \scriptsize{29.45} & \scriptsize{54.49} & \scriptsize{54.19} & \scriptsize{27.81} & \scriptsize{39.93}
% \\\hline

% \scriptsize{EBSeg \cite{shan2024open}} & \scriptsize{CLIP ViT-B/16} & \scriptsize{27.24} & \scriptsize{25.59} & \scriptsize{50.75} & \scriptsize{51.09} & \scriptsize{26.68} & \scriptsize{36.27} 
% \\\hline

% \scriptsize{RSKT-Seg \cite{li2025exploring}} & \scriptsize{CLIP ViT-B/16} & \scriptsize{35.38} & \scriptsize{37.70} & \scriptsize{56.74} & \scriptsize{68.48} & \scriptsize{35.95}  & \scriptsize{46.85} 

% \\\hline

% \scriptsize{GSNet \cite{ye2025towards}} & \scriptsize{CLIP ViT-B/16} & \scriptsize{35.20} & \scriptsize{36.94} & \scriptsize{56.96} & \scriptsize{55.03} & \scriptsize{32.40} & \scriptsize{42.37} 

% \\\hline

% \scriptsize{FGA-Seg \cite{li2025fgaseg}} & \scriptsize{CLIP ViT-B/16} & \scriptsize{25.95} & \scriptsize{32.77} & \scriptsize{51.55} & \scriptsize{51.62} & \scriptsize{40.57}  & \scriptsize{40.49} 
% \\\hline

% \scriptsize{SegEarth-OV \cite{li2025segearth}} & \scriptsize{CLIP ViT-B/16} & \scriptsize{28.88} & \scriptsize{18.53} & \scriptsize{45.05} & \scriptsize{17.57} & \scriptsize{24.17}  & \scriptsize{26.84} 
% \\\hline

% \scriptsize{MM-OVSeg (ours)}& \scriptsize{CLIP ViT-B/16}  & \scriptsize{\bf 36.61} & \scriptsize{\bf 40.21} & \scriptsize{\bf 57.65} & \scriptsize{\bf 73.11} & \scriptsize{\bf 42.64}  & \scriptsize{\bf 50.04} 

% \\\hline
% \end{tabular}}
% \end{table*}



%--------------------------------

% In this section, we first introduce the OpenEarthMap-SAR \cite{xia2025openearthmap}, PIE-RGB-SAR \cite{ZHANG2024574}, DDHR-SK \cite{ren2022dual} and DDHR-CH \cite{ren2022dual} datasets and their experimental settings in Section 4.1. Then, we report our results on these datasets and compare our model with several existing methods in Section 4.2. Finally, we provide ablation analyses on the DINO distillation and multimodal feature fusion strategies proposed in this paper and justify their contributions in Section 4.3.
%-------------------------------------------------------------------------
\subsection{Datasets and Settings}

\subsubsection{Experimental Setups}
We comprehensively evaluate MM-OVSeg across multiple multimodal RS datasets under diverse weather and domain conditions. Our evaluation encompasses (1) \textbf{clear-sky vs. cloudy weather}, (2) \textbf{real vs. synthetic cloud} cover with varying opacity (\textbf{thin vs. thick}), and (3) \textbf{intra-domain and cross-domain} generalization.

% {\bf OpenEarthMap-SAR.} The OpenEarthMap-SAR dataset \cite{xia2025openearthmap} comprises 1.5 million segmented tiles (1024 × 1024 pixels) derived from 5,033 aerial and satellite images spanning 35 regions in Japan, France, and the United States. The dataset encompasses eight land-cover categories: bareland, rangeland, developed space, road, tree, water, agriculture land and building. These land-cover masks are either partially manually annotated or fully pseudo-labeled, with a ground sampling distance (GSD) of 0.15–0.5 m. In accordance with the dataset partitioning for the semantic segmentation task in \cite{xia2025openearthmap}, the training set consists of 4,333 RGB-SAR image pairs with pseudo-semantic labels, while the test set comprises 490 RGB-SAR image pairs with manually annotated semantic labels. To simulate extreme weather conditions, we apply the SatelliteCloudGenerator \cite{rs15174138} to the RGB images of OpenEarthMap‑SAR \cite{xia2025openearthmap}, synthesizing thin and thick cloud occlusions and yielding two derived subsets: OpenEarthMap‑SAR (thin cloud) and OpenEarthMap‑SAR (thick cloud).

\textbf{OpenEarthMap-SAR} \cite{xia2025openearthmap} comprises 1.5 million segmented tiles (1024 × 1024 pixels) collected from aerial and satellite imagery over 35 regions in Japan, France, and the United States, with a ground sampling distance (GSD) of 0.15–0.5 m. Eight land-cover categories are annotated. Following the official split, we use 4,333 RGB–SAR image pairs for training and 490 pairs for testing.
Since the dataset contains only clear-sky imagery, we apply SatelliteCloudGenerator \cite{rs15174138} to synthesize cloud cover, producing two variants: \textbf{OEM-thin} and \textbf{OEM-thick}.
Training classes include \textit{Bareland, Rangeland, Developed space, Tree}, and \textit{Agriculture land}, while testing additionally includes novel classes \textit{Road, Water}, and \textit{Building}.

% SAR samples are sourced from Umbra and acquired in Spotlight mode, with spatial resolution (GSD) ranging from 0.15 to 0.5 m. The optical data include red, green, and blue bands, while the SAR data primarily comprise amplitude backscatter in VV or HH polarization. To ensure precise cross-modal alignment, paired optical–SAR tiles were manually co-registered by multiple experts and cross-verified to meet stringent quality standards.

% {\bf PIE-RGB-SAR.} The dataset \cite{ZHANG2024574} comprises multimodal image pairs sourced from the Pearl River Delta, China. RGB images from Google Satellite serve as the primary source, while SAR images from the GF3 satellite’s ultra-fine stripe mode provide complementary information to assist in land type identification for each pixel. The spatial resolutions of the RGB and SAR images are approximately 0.5 meters and 3 meters, respectively. The dataset is annotated into six categories: city, road, water, forest, farmland, and others. The distribution is imbalanced, with 30\% city, 3\% road, 7\% water, 42\% forest, 10\% farmland, and 8\% other. The RGB-SAR image pairs are cropped to a uniform size of 256x256, resulting in a total of 4,865 images. Following the train/test partitioning outlined in \cite{ZHANG2024574}, the training set comprises 2,433 images, while the test set contains 2,432 images.

\textbf{PIE-RGB-SAR} \cite{ZHANG2024574} contains multimodal image pairs from the Pearl River Delta, China, with RGB images sourced from Google Satellite and SAR images from the GF-3 satellite’s ultra-fine stripe mode. The RGB and SAR images have approximate GSD of 0.5 m and 3 m, respectively. All pairs are cropped to 256 × 256 pixels, yielding 4,865 samples (2,433 for training and 2,432 for testing). Two tracks are officially provided: \textbf{PIE-clean} (cloud-free) and \textbf{PIE-cloud} (cloudy). We use training classes \textit{Backroad, City, Forest}, and \textit{Farmland}, and define \textit{Road} and \textit{Water} as novel test classes.

% Given the absence of pixel values for the ‘others' category in both the corresponding RGB and SAR modalities, the semantic labels for this category were excluded from our open vocabulary semantic segmentation experiments. 

% {\bf DDHR-SK and DDHR-CH.} The dataset \cite{ren2022dual} consists of five multimodal image groups sourced from three regions: Xi’an and Dongying in China, and Pohang in South Korea. Following \cite{ZHANG2024574}, our experiments adopt the cloudy subsets from the Pohang and Xi’an regions, denoted DDHR‑SK and DDHR‑CH, respectively. The official data splits for DDHR‑SK are publicly available. These two datasets encompass five classes: city, road, forest, water, and farmland. The RGB image sourced from the GF‑2 satellite is synthetically clouded using the GNU Image Manipulation Program (GIMP) to simulate cloud cover. The SAR image captured by the GF‑3 satellite is resampled to a resolution of 1 meter. Both RGB and SAR images are cropped to 256 × 256 pixels. In total, there are 3,087 training images and 3,086 validation images in the DDHR-SK dataset. All images in the DDHR-CH dataset are treated as the test set.

\textbf{DDHR} \cite{ren2022dual} includes RGB images from the GF-2 satellite, synthetically clouded using the GNU Image Manipulation Program (GIMP) software, paired with SAR images from GF-3 resampled to 1 m resolution. Both modalities are cropped to 256 × 256 pixels.
The dataset contains five subsets; we use two: \textbf{DDHR-SK} (Pohang, South Korea) and \textbf{DDHR-CH} (Xi’an, China).
For DDHR-SK, we follow the official split with 3,087 training and 3,086 validation images. DDHR-CH is used entirely for cross-domain testing.
Five classes are annotated, among which \textit{Forest, City}, and \textit{Farmland} are used for training, and \textit{Road} and \textit{Water} are treated as novel classes in testing.

{\bf Evaluation Protocol.} Table \ref{tab:datasets} summarizes the evaluation setups across the datasets described above.
We report mean Intersection over Union (mIoU) as the primary metric for evaluation of semantic segmentation performance.
% We adopt two protocols: (i) intra‑dataset evaluation, where the training and test sets are drawn from the same dataset (applied to the first four datasets), and (ii) cross‑dataset evaluation, where training and testing originate from different datasets. Specifically, we assess the generalization ability of our MM-OVSeg model by training on the DDHR-SK \cite{ren2022dual} dataset and testing on the DDHR‑CH \cite{ren2022dual} dataset. Table \ref{tab:table1} presents the open‑vocabulary setting (training and unseen categories) and the statistics of the training and test splits used in our experiments.


\subsubsection{Implementation Details}

% Our implementation is built on PyTorch \cite{paszke2019pytorch} and Detectron2 \cite{wu2019detectron2}. During cross-modal unification, we set the batch size to 8 and train DINO v1 \cite{caron2021emerging} model using the AdamW \cite{loshchilov2017decoupled} optimizer with the initial learning rate of 3e-4. We adopt OpenAI pretrained CLIP \cite{openclip2022} (ViT-B/16) model and fine‑tune it \cite{openclip2022} with a learning rate of 2e‑6. All remaining modules are randomly initialized and optimized with a learning rate of 2e‑4. We set the batch size to 8, and train models for 120,000 iterations using the AdamW \cite{loshchilov2017decoupled} optimizer with the initial learning rate of 2.5e-4, weight decay of 1e-4. All experiments are conducted on a NVIDIA RTX A100 GPU.

% Our implementation is based on PyTorch \cite{paszke2019pytorch} and Detectron2 \cite{wu2019detectron2}. We use ViT‑B/16 as backbone for both CLIP and DINO models. For pre-trained paramters, we adopt official OpenCLIP \cite{openclip2022} and DINO v1 \cite{caron2021emerging}. When training for CMU, the batch size is 8, optimized with the AdamW \cite{loshchilov2017decoupled} optimizer and an initial learning rate of $3\times10^{-4}$, and a weight decay of $1\times10^{-4}$. For full MM-OVSeg Training. We use a learning rate of $2\times10^{-6}$. All new introduced parameters are randomly initialized. The full model is trained for 120,000 iterations using AdamW with an initial learning rate of $2.5\times10^{-4}$ and a batch size of 8.
% All experiments are conducted on a single NVIDIA RTX A100 GPU (80 GB).

We implement MM-OVSeg in PyTorch \cite{paszke2019pytorch} using Detectron2 \cite{wu2019detectron2} for the segmentation pipeline. Both CLIP and DINO components use a ViT-B/16 backbone. Pretrained weights are taken from OpenCLIP \cite{openclip2022} and DINO v1 \cite{caron2021emerging}.
(1) CMU training: We train the SAR DINO encoder with a batch size of 8 using AdamW \cite{loshchilov2017decoupled}. The learning rate is set to $3\times10^{-4}$ with a weight decay of $1\times10^{-4}$. The RGB DINO encoder remains frozen. 
(2) Full MM-OVSeg training:
All newly introduced parameters are initialized randomly. We fine-tune the model for 120k iterations using AdamW with a batch size of 8 and an initial learning rate of $2.5\times10^{-4}$. The CLIP encoders are trained with a smaller learning rate of $2\times10^{-6}$ to preserve their pretrained alignment. All experiments are conducted on a single NVIDIA RTX A100 GPU (80 GB).

% \subsubsection{\textcolor{red}{Baseline Methods}}

% Since the proposed MM-OVSeg is a multimodal fusion method and there is no previous OVS method designed for cloudy RGB image, we select 6 state-of-the-art baselines for comparison:

% \textbf{(1) OVS Models:} CAT-Seg \cite{cho2024catseg}, EBSeg \cite{shan2024open} and FGA-Seg \cite{li2025fgaseg}.

% \textbf{(2) Training-free OVRS Model:} SegEarth-OV \cite{li2025segearth}.

% \textbf{(3) OVRS Models:} GSNet \cite{ye2025towards}.

% and RSKT-Seg \cite{li2025exploring}.

\subsubsection{Baselines and Comparison Methods}
Since the proposed MM-OVSeg is the first multimodal fusion framework for OVS in RS, we compare it with six state-of-the-art single-modality OVS models.
These include
1) OVS models in the natural image domain: CAT-Seg \cite{cho2024catseg}, EBSeg \cite{shan2024open}, and FGA-Seg \cite{li2025fgaseg};
2) OVS models in the RS domain: GSNet \cite{ye2025towards}; and
3) a training-free RS OVS model: SegEarth-OV \cite{li2025segearth}, used as a reference baseline.
%-------------------------------------------------------------------------
\subsection{Main Result}

Table \ref{tab:table2} presents a quantitative comparison between MM-OVSeg and recent state-of-the-art methods across all benchmark datasets. mIoU is reported for each dataset and their overall mean, \textcolor{red}{with the statistics of per-class results provided in the Figure \ref{fig:figzhu}.} Overall, MM-OVSeg achieves the highest average performance, reaching 51.7\% over six benchmarks, while the second-best method, GSNet, obtains 45.6\%. This substantial improvement highlights the effectiveness of the proposed multimodal fusion framework in advancing open-vocabulary segmentation within the remote sensing domain. 
% \textcolor{red}{We also report the quantitative comparison between MM-OVSeg and recent state-of-the-art methods based on ViT-L/14 backbone. Please refer to Appendix A for more details.} 
Key observations are summarized below.

% \textcolor{red}{51.7\% mIoU with ViT-B/16 backbone and XXX \% mIoU with ViT-L/14 backbone, respectively}

%--------------------------------------
\begin{figure*}[ht]
\centering
\includegraphics[width=\linewidth]{sec/fig3.pdf}
%\begin{minipage}{0.8\textwidth}
\caption{{\bf Visualization of Open-Vocabulary Semantic Segmentation Results.}  From left to right: cloudy RGB image, SAR image, ground truth (GT), segmentation results of CAT-Seg \cite{cho2024catseg}, EBSeg \cite{shan2024open}, GSNet \cite{ye2025towards}, SegEarth-OV \cite{li2025segearth} and our MM-OVSeg. \ding{172}: PIE-cloud→PIE-cloud; \ding{173}: DDHR-SK→DDHR-SK; \ding{174}: OEM-thick→OEM-thick; \ding{175}: OEM-thin→OEM-thin; \ding{176}: PIE-clean→PIE-clean; \ding{177}: DDHR-SK→DDHR-CH. Please refer to Table 1 for dataset details.}
%\end{minipage}
\label{fig:fig3}
\end{figure*}

%--------------------------------

\textbf{Cross-weather robustness.} MM-OVSeg delivers consistently strong performance under various cloudy and hazy conditions. Its adaptive fusion mechanism effectively exploits the cloud-penetrating capability of SAR while dynamically weighting RGB and SAR cues according to scene quality. As a result, MM-OVSeg achieves the best performance in all weather scenarios. Notably, even on the clear-sky benchmark (\ding{176}: PIE-clean → PIE-clean), where SAR contributions are less critical, MM-OVSeg still surpasses GSNet by 2.5\% mIoU.
% MM-OVSeg maintains consistently strong performance under both clear-sky and cloudy conditions. While SAR imagery contributes most under cloud-covered settings due to its cloud-penetrating capability, our adaptive fusion mechanism allows the model to dynamically balance RGB and SAR information. As a result, MM-OVSeg achieves the best results in all weather scenarios and still exceeds GSNet by 2.5\% mIoU on clear-sky dataset (\ding{176}: PIE-clean→PIE-clean).

\textbf{Cloud-type and cloud-cover variability.} Across both real and synthetic clouds, including thin, thick, and mixed layers, MM-OVSeg yields stable segmentation accuracy. This indicates that the model learns to exploit complementary spectral and structural cues from the two modalities rather than overfitting to specific cloud patterns, confirming the flexibility of our fusion strategy.

\textbf{Domain generalization.} To evaluate cross-domain robustness, we train on DDHR-SK and test on DDHR-CH (\ding{177}: DDHR-SK→DDHR-CH), which represent distinct geographic regions. As expected, all \textcolor{red}{training-required} methods experience performance degradation comparing intra-domain testing (\ding{173}: DDHR-SK→DDHR-SK), reflecting significant domain discrepancy. Nevertheless, MM-OVSeg maintains a clear margin over all competitors, demonstrating leading adaptability to unseen regions.

\textbf{Qualitative analysis.}
Figure~\ref{fig:fig3} provides visual comparisons. Previous models are highly sensitive to cloud interference: thick clouds often cause misclassification, and even thin haze layers can distort predictions. In contrast, MM-OVSeg produces coherent and accurate segmentations by adaptively leveraging both optical and SAR information. Moreover, the model correctly identifies novel categories that are unseen during training, validating its strong text-feature alignment. Additional qualitative results are provided in the appendix.

% {\bf Evaluation on OpenEarthMap-SAR.} Table \ref{tab:table2} (line 3 and 4) reports the open-vocabulary semantic segmentation results on the OpenEarthMap-SAR dataset. \textcolor{red}{The qualitative results for each category can be found in Appendix Table 1-2.} Our MM-OVSeg consistently outperforms CAT-Seg \cite{cho2024catseg}, EBSeg \cite{shan2024open}, and SegEarth-OV \cite{li2025segearth} on both thick‑cloudy and thin‑cloudy subsets. It establishes a new state-of-the-art results with mIoU of 36.6 and 40.2 on the thick‑cloudy and thin‑cloudy subsets, respectively. Further, our method achieves the best performance in 4 of 8 categories, including two unseen categories (water and building) and bareland category, on thick‑cloudy subset. Our method also achieves the best performance under 5 out of 8 categories on thin‑cloudy subset, including all unseen categories and bareland category. The improvement stems from that our MM-OVSeg model can capture the effectively spatial information from the SAR images, leveraging SAR backscatter patterns to recover semantics lost to cloud occlusions in RGB imagery.

% To provide an intuitive comparison, we visualize two segmentation results on the OpenEarthMap-SAR (thin cloud) and OpenEarthMap-SAR (thick cloud) datasets, as shown in Figure \ref{fig:fig3}. It can be seen that our MM-OVSeg accurately segments most objects and produces sharper object boundaries than the baselines. Notably, in the first row of Figure \ref{fig:fig3}, substantial portions of the water category are misclassified as tree or agricultural land by CAT-Seg \cite{cho2024catseg}, EBSeg \cite{shan2024open}, SegEarth-OV \cite{li2025segearth} and GSNet \cite{ye2025towards}, but correctly classified by our MM-OVSeg. 

% To further evaluate the effectiveness of the feature aggregation strategy (DEF module) of MM-OVSeg, we visualize the cost maps of CLIP image encoder, DINO encoders and MM-OVSeg, as shown in Figure \ref{fig:fig4}. It can be seen that DINO encoders provide complementary information for CLIP image encoder, achieving better performance for both training categories and unseen categories under cloudy conditions.

% {\bf Evaluation on PIE-RGB-SAR.} Table \ref{tab:table2} (line 5) shows the open-vocabulary semantic segmentation results on the PIE-RGB-SAR dataset. As shown in Table \ref{tab:table2}, it can seen that our MM-OVSeg outperforms all existing methods, achieving the mIoU score of 57.7. Further, our MM-OVSeg surpasses the state-of-the-art method GSNet \cite{ye2025towards} by 0.7\% in mIoU and achieves a consistent performance improvement in 2 out of 6 categories, including a unseen category (water) and farmland category. We further visualize qualitative results from the PIE-RGB-SAR dataset. As demonstrated in the third row of Figure \ref{fig:fig3}, the unseen water category poses difficulties for competing models \cite{cho2024catseg,shan2024open,ye2025towards,li2025segearth}, but our method accurately identifies and delineates most water areas. \textcolor{red}{The qualitative results for each category can be found in Appendix Table 3.}

% Compared with the other datasets, our gains on PIE‑RGB‑SAR are below the average mIoU improvement (i.e. 3.19\%), largely because only a small fraction of the RGB images (≈25\%) contain thin‑cloud occlusions, reducing the benefit of SAR complementation.

%-------- table2 ------------
% \begin{table*}[t]

% \centering
% \caption{\label{tab:table2}{{\bf Open-Vocabulary Semantic Segmentation Results on the PIE-RGB-SAR Dataset.} Mean IoU (\%) is used as the evaluation metric.}}

% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|cccccc|}
% \hline

% \scriptsize{\bf Method} & \scriptsize{\bf mIoU} & \scriptsize{Other} & \scriptsize{City} & \scriptsize{Road} & \scriptsize{Water} & \scriptsize{Forest} & \scriptsize{Farmland}   


% \\\hline
% \scriptsize{FGA-Seg \cite{li2025fgaseg}} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} 
% \\

% \scriptsize{CAT-Seg \cite{cho2024catseg}} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} 
% \\

% \scriptsize{EBSeg \cite{shan2024open}} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} 

% \\

% \scriptsize{RSKT-Seg \cite{li2025exploring}} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} 

% \\

% \scriptsize{GSNet \cite{ye2025towards}} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} 

% \\\hline
% \scriptsize{MMEarth-OVRS (ours)} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} & \scriptsize{} &  \scriptsize{\bf }

% \\\hline
% \end{tabular}}
% \end{table*}
%--------------------------------

% {\bf Evaluation on DDHR-SK.} Table \ref{tab:table3} (line 6) presents the segmentation results on the DDHR-SK dataset. Compared to the state‑of‑the‑art baseline GSNet \cite{ye2025towards}, our model achieves the most remarkable improvement of 18.1\% in terms of mIoU. These results demonstrate the effectiveness of our model in overcoming cloud occlusions for open‑vocabulary remote sensing segmentation. Moreover, the qualitative examples in Figure \ref{fig:fig3} (rows 4) indicate consistent improvements across category types: our method enhances segmentation of the seen city, forest and farmland classes. \textcolor{red}{The qualitative results for each category can be found in Appendix Table 4.}

% {\bf Cross-domain Generalization Test.} To assess cross‑domain generalization ability, we evaluate our MM‑OVSeg on the entire DDHR‑CH dataset without any fine‑tuning or additional training. Specifically, we adopt the training set of DDHR-SK dataset to train our MM-OVSeg model, and then evaluate our model on the entire DDHR-CH dataset. According to Table \ref{tab:table3} (line 7), our approach surpasses FGA‑Seg by 2.0\% in terms of mIoU, confirming its robustness and generalization under cloud occlusions across diverse remote sensing scenes. As demonstrated in the fifth row of Figure \ref{fig:fig3}, the farmland category poses difficulties for competing models \cite{cho2024catseg,shan2024open,ye2025towards,li2025segearth}, but our method accurately segments whole farmland areas. \textcolor{red}{The qualitative results for each category can be found in Appendix Table 5.}

% {\bf Cloud-free Segmentation.} We additionally evaluate our MM-OVSeg on the cloud‑free subset of the PIE‑RGB‑SAR dataset to access its effectiveness beyond occluded scenarios. According to Table \ref{tab:table2} (line 8), MM‑OVSeg achieves state‑of‑the‑art results under cloud‑free conditions, indicating that our multimodal feature fusion strategy (DEF) remains robust and effective under cloud‑free conditions. \textcolor{red}{The qualitative results for each category can be found in Appendix Table 6.}


%-------------- Table 3 ------------------
\begin{table}[t]
    \renewcommand{\arraystretch}{1.15}
    \resizebox{\linewidth}{!}{%
    \centering
    % \footnotesize
    \begin{tabular}{l|ccccc|c}
    \toprule
       Model Variant & Forest & City & Farmland & Road & Water & mIoU \\
    \midrule
       MM-OVSeg & 87.3 & 86.8 & 85.6 & 21.2 & 84.8 & 73.1 \\
       \textit{w/o} CMU  & 57.2 & 83.7 & 81.2 & 16.8 & 81.4 & 64.1 \\
       \textit{w/o} CMU\&DEF  & 80.0 & 90.3 & 79.0  & 6.8 & 19.1 & 55.0 \\
    \bottomrule
    \end{tabular}}
    \caption{Ablation study of MM-OVSeg on the DDHR-SK→DDHR-SK cloud segmentation task. The proposed DEF module enables effective multimodal fusion, substantially improving over the single-modality baseline. In combination with CMU, the full model achieves the best performance, demonstrating that CMU and DEF are complementary.}
    \label{tab:ablation}
\end{table}

%-------------------------------------------------------------------------
\subsection{Ablation Studies}

We conduct ablation experiments to analyze the contribution of each component in MM-OVSeg to open-vocabulary segmentation. All experiments are performed on the DDHR-SK dataset, and results are summarized in Table~\ref{tab:ablation}. The baseline model, which uses only optical data without the proposed Cross-Modal Unification (CMU) or Dual-Encoder Fusion (DEF) modules, achieves 55.0\% mIoU, revealing the limitation of single-modality segmentation. Introducing the DEF module leads to a clear improvement by 9.1\%, confirming the effectiveness of multimodal feature integration between RGB and SAR data. Finally, incorporating both CMU and DEF yields the full MM-OVSeg, which achieves the best performance to 73.1\%. These results demonstrate that CMU and DEF are complementary: CMU effectively aligns SAR features with RGB representations, while DEF fuses them adaptively for robust multimodal segmentation.


\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{Figures/Fig-vis-DEF.pdf}
\caption{Visualization of different stages in multimodal fusion within DEF. DEF produces finer spatial localization and stronger alignment between dense and global visual features and text representations.}
%\end{minipage}
\label{fig:fig4}
\end{figure}

\subsection{Discussions}

\subsubsection{Feature Visualization and Analysis of DEF}

To better understand how DEF integrates representations from different foundation models and modalities, we visualize the intermediate feature maps generated at various stages of the fusion process.
As illustrated in Figure \ref{fig:fig4}, we show (1) the input RGB image for reference, (2) the global visual feature $z_{\text{rgb}}$ extracted by the CLIP visual encoder, (3) the multimodal dense feature $f_d$ obtained from DINO and DINO-SAR, and (4) the final fused representation $h_{\text{fuse}}$, which combines dense RGB and SAR features with global CLIP visual and text embeddings.
We use text prompts corresponding to two seen categories (Rangeland, Tree) and two unseen categories (Water, Road), and visualize their attention heatmaps.

The results reveal several insights.
First, the CLIP visual encoder is relatively less affected by cloud interference than DINO, but its attention maps remain coarse because it primarily captures global semantics.
Second, CLIP and DINO exhibit complementary attention patterns—regions highlighted strongly by one are often suppressed by the other—indicating that their feature spaces encode different but synergistic cues.
Finally, the fused representation $h_{\text{fuse}}$ provides much finer spatial localization and better alignment with text prompts, accurately highlighting both seen and unseen categories.
These visualizations confirm that DEF effectively unifies dense and global representations across modalities, leading to improved semantic correspondence and robustness under cloudy conditions.

 % In this section, we employ three comparative experiments to verify the effectiveness of the proposed CMU, DEF module and InfoNCE \cite{oord2018representation} loss function adopted in the CMU module. The DDHR-SK dataset is chosen for evaluation. To demonstrate the effectiveness of our CMU and DEF strategy, we construct two ablated variants: (i) Ours‑singleDINO removes both modules and directly fuses DINO‑RGB local features with local CLIP features; (ii) Ours‑multiDINO‑pretrain only removes CMU module but employs two frozen DINO encoders pretrained on LandDiscover50K \cite{ye2025towards} dataset to extract spatial features from RGB and SAR, respectively.

\begin{table}[t]
    \setlength{\tabcolsep}{20pt}
    \centering
    \begin{tabular}{l|c}
    \toprule
        Loss type & mIoU \\
    \midrule
        \textit{baseline} & 64.1 \\
        MSE & 67.7 \\
        L1 & 69.0 \\
        InfoNCE & \textbf{73.1} \\
    \bottomrule
    \end{tabular}
    \caption{Effect of different loss functions on CMU performance.}
    \label{tab:losses}
\end{table}


% \begin{table}[t] %\color{red} % 删掉\color{red}即可，不加resizebox
%     \footnotesize % 这里整体调字体
%     \centering
%     \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%     \begin{tabular}{l|cc|c|c}
%     \toprule
%         Method & CMU & DEF & Loss & mIoU \\ 
%     \midrule
%         Ours-singleDINO & $\times$ & $\times$ & InfoNCE \cite{oord2018representation} & 55.0  \\

%     \midrule
%         Ours-multiDINO-pretrain & $\times$ & $\surd$ & InfoNCE \cite{oord2018representation} & 64.0  \\

%     \midrule
%         Ours & \tabincell{c}{\scriptsize{$\surd$} \\ \scriptsize{$\surd$}\\ \scriptsize{$\surd$}} & \tabincell{c}{\scriptsize{$\surd$} \\ \scriptsize{$\surd$}\\ \scriptsize{$\surd$}} & \tabincell{c}{\scriptsize{MSE \cite{gauss1809}} \\ \scriptsize{L1 \cite{koenker1978regression}} \\ \scriptsize{InfoNCE \cite{oord2018representation}}} & \tabincell{c}{\scriptsize{67.7} \\ \scriptsize{69.0}\\ \scriptsize{\bf 73.1}}  \\ 
%     \bottomrule
%     \end{tabular}
%     \caption{Ablation Results on the DDHR-SK Dataset. Mean IoU (\%) is used as the evaluation metric. The CMU and DEF denote the proposed CMU and DEF modules. ‘$\times$' refers to the absence of the corresponding module, while ‘$\surd$' indicates the existence of the corresponding module.}
%     \label{tab:table3}
% \end{table}
 %-------- table3 ------------
% \begin{table}[t]
% \centering
% \newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
% \caption{\label{tab:table3}{{\bf Ablation Results on the DDHR-SK Dataset.} Mean IoU (\%) is used as the evaluation metric. The CMU and DEF denote the proposed CMU and DEF modules. ‘--' refers to the absence of the corresponding module, while ‘$\surd$' indicates the existence of the corresponding module.}}
% % \resizebox{\linewidth}{!}{
% \begin{tabular}{|c|cc|c|c|}
% \hline

% \scriptsize{\bf Method} & \scriptsize{\bf CMU} & \scriptsize{\bf DEF} & \scriptsize{\bf Loss} & \scriptsize{mIoU}   


% \\\hline
% \scriptsize{Ours-singleDINO} & \scriptsize{$\times$} & \scriptsize{$\times$} & \scriptsize{InfoNCE \cite{oord2018representation}} & \scriptsize{55.03}
% \\\hline

% \scriptsize{Ours-multiDINO-pretrain} & \scriptsize{$\times$} & \scriptsize{$\surd$} & \scriptsize{InfoNCE \cite{oord2018representation}} & \scriptsize{64.08} 

% \\\hline
% \scriptsize{Ours} & 
% \tabincell{c}{\scriptsize{$\surd$} \\ \scriptsize{$\surd$}\\ \scriptsize{$\surd$}} & \tabincell{c}{\scriptsize{$\surd$} \\ \scriptsize{$\surd$}\\ \scriptsize{$\surd$}} & 
% \tabincell{c}{\scriptsize{MSE \cite{gauss1809}} \\ \scriptsize{L1 \cite{koenker1978regression}} \\ \scriptsize{InfoNCE \cite{oord2018representation}}} & 
% \tabincell{c}{\scriptsize{67.74} \\ \scriptsize{69.06}\\ \scriptsize{\bf 73.11}}

% \\\hline
% \end{tabular}
% % \end{tabular} }
% \end{table}
%--------------------------------


%  \subsubsection{The DEF Strategy}

% The DEF strategy extends the unimodal OVRS pipeline to handle multimodal inputs and improves accuracy. As reported in Table \ref{tab:table3} (rows 3 and 6), Ours‑multiDINO‑pretrain surpasses Ours‑singleDINO by 9.0\% mIoU, achieving improvements in 4 out of 5 categories, including all unseen categories (road and water) and two training categories (forest and farmland).

 \subsubsection{Loss Design in CMU}

We analyze the impact of different loss functions used in the Cross-Modal Unification (CMU) stage. Specifically, we compare MSE loss, L1 loss, and InfoNCE loss to evaluate how they affect the feature alignment between SAR and RGB representations in the DINO encoders. The model without CMU is also included as a baseline for reference. As shown in Table \ref{tab:losses}, all three loss functions yield notable improvements over the baseline, confirming the effectiveness of the CMU framework. Among them, the InfoNCE loss achieves the highest performance, surpassing both MSE and L1 losses by a clear margin.

% \begin{table}[t]
%     \centering
%     \begin{tabular}{c|cc|c}
%     \toprule
%         Method & CLIP & DINO & mIoU\\
%     \midrule
%         1 & \xmark & \xmark & 64.1 \\
%         2 & \cmark & \xmark & 65.4 \\
%         3 & \xmark & \cmark & \textbf{73.1} \\
%         4 & \cmark & \cmark & 66.5 \\
%     \bottomrule
%     \end{tabular}
%     \caption{Effect of different distilled backbones on the DDHR-SK→DDHR-SK cloud segmentation task.}
%     \label{tab:distill}
% \end{table}

 % \textcolor{red}{\subsubsection{Distilled  Backbone Design in CMU} \label{sec:distillation}} 

 % \textcolor{red}{We further analyze the impact of different distilled backbones used in the Cross-Modal Unification (CMU) stage. Specifically, we compare the distillation of CLIP and DINO backbone to evaluate how they affect the feature alignment between SAR and RGB representations. The model without CMU is also included as a baseline for reference. As shown in Table \ref{tab:distill}, all distilled backbones yield notable improvements over the baseline, further confirming the effectiveness of the CMU framework. Among them, DINO‑backbone distillation yields larger gains than CLIP‑backbone distillation. Moreover, distilling the CLIP backbone reduces the contribution of DINO-backbone distillation to the final results.}

% When distilling DINO encoders, a contrastive InfoNCE \cite{oord2018representation} loss is advantageous over MSE \cite{gauss1809} or L1 \cite{koenker1978regression} as it explicitly maximizes agreement between positive pairs while repelling negatives, yielding more discriminative, semantically aligned representations. To demonstrate the effectiveness of InfoNCE loss during cross-modal distillation, we conduct three comparative experiments to quantify the contribution of the InfoNCE strategy. According to Table \ref{tab:table3} (rows 4-6), InfoNCE improves mIoU by 4.1\% over L1 and by 5.4\% over MSE. \textcolor{red}{The qualitative results for each category can be found in Appendix Table 7.}
%-------------------------------------------------------------------------

% \subsubsection{\textcolor{red}{The CMU Strategy}}

% \textcolor{red}{The CMU strategy not only enhances the DINO encoder’s ability to extract effectively spatial features from SAR images and boosts overall accuracy. Table \ref{tab:table3} reports that our model outperforms Ours‑multiDINO‑pretrain by incorporating CMU module. Specifically, the CMU strategy contributes ${\rm{9.1\% }}$ in terms of mIoU, and achieves better performance in 4 out of 5 categories, including all unseen categories (road and water) and two training categories (forest and farmland).}

